StyleCLIPDraw: Coupling Content and Style in Text-to-Drawing Translation

Generating images that fit a given text description using machine learning has improved greatly with the release of technologies such as the CLIP image-text encoder model; however, current methods lack artistic control of the style of image to be generated. We present an approach for generating styled drawings for a given text description where a user can specify a desired drawing style using a sample image. Inspired by a theory in art that style and content are generally inseparable during the creative process, we propose a coupled approach, known here as StyleCLIPDraw, whereby the drawing is generated by optimizing for style and content simultaneously throughout the process as opposed to applying style transfer after creating content in a sequence. Based on human evaluation, the styles of images generated by StyleCLIPDraw are strongly preferred to those by the sequential approach. Although the quality of content generation degrades for certain styles, overall considering both content \textit{and} style, StyleCLIPDraw is found far more preferred, indicating the importance of style, look, and feel of machine generated images to people as well as indicating that style is coupled in the drawing process itself. Our code (https://github.com/pschaldenbrand/StyleCLIPDraw), a demonstration (https://replicate.com/pschaldenbrand/style-clip-draw), and style evaluation data (https://www.kaggle.com/pittsburghskeet/drawings-with-style-evaluation-styleclipdraw) are publicly available.

==> discussion-saved.tex <==

\section{Discussion}

\subsection{Degrading Content Results}

StyleCLIPDraw was favored to the baseline decoupled approach when both style \textit{and} content were considered and when just style was considered, but it was inferior when just content was considered. 
We hypothesized that the choice of style image affected the content of the results.  Since StyleCLIPDraw applied the style far more that the baseline, it could be true that the style hurt the appearance of the content of the image more than the baseline.

We wanted to compare the agreement on realism of a style image and the appearance of content.
We asked AMT workers to rate the 8 style images used in our study from simplest to most detailed. ``very detailed" got a score of 2, ``simple" was -1, ``neutral" was 0, etc. We then compared the standard deviation of these scores to the results from the content survey broken down by style image. A high standard deviation indicated that participants did not agree on how realistic the style image was.  A high percentage indicated that the StyleCLIPDraw images of that style had great content compared to the baseline. In Figure \ref{fig:std_realism}, there is a strong, positive correlation between the divided opinion on realism of the image and the appearance of content in the image.



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/std_realism.png}
    \caption{Each point represents a style image. The y axis is the percentage of times StyleCLIPDraw was chosen over the baseline in terms of style for that style image, and the x axis is the standard deviation in the rating on realism/detailed/simple the style image was.}
    \label{fig:std_realism}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/mean_realism.png}
    \caption{Each point represents a style image. The y axis is the percentage of times StyleCLIPDraw was chosen over the baseline in terms of style for that style image, and the x axis is the average in the rating on realism/detailed/simple the style image was.}
    \label{fig:mean_realism}
\end{figure}

We also hypothesized that the additional loss in StyleCLIPDraw's optimization made results in terms of content worse.   Adding style as a loss is a way to constrain the number of acceptable solutions: within the space of all drawings, there exists a subset that fit a given text description.  Within that set is a smaller set that fit the description AND the given style image. See Figure \ref{fig:style_constraint}.  To test this hypothesis, we measured the average style and content losses between three optimizations: all content loss (equivalent to CLIPDraw),  all style loss, and style and content loss (StyleCLIPDraw).  These results are shown in Table \ref{tab:best_losses}.  Optimizing for just content reached better content losses than optimizing for both content and style.

\begin{figure}[h]
    \centering
    \includegraphics[width=7cm]{images/style_constraint.png}
    \caption{Caption}
    \label{fig:style_constraint}
\end{figure}

\begin{table}[h]
\centering
\begin{tabular}{lp{1.8cm}p{1.95cm}p{2.25cm}}
\toprule
  & Style Only & Content Only \newline (CLIPDraw) & Style \& Content \newline (StyleCLIPDraw) \\
\midrule
Content \\Loss & -0.21 $\pm$ 0.03 & \textbf{-0.39  $\pm$ 0.04} & -0.35  $\pm$ 0.04 \\
Style \\Loss   & 1.60  $\pm$ .33  & 2.04  $\pm$ 0.20  & \textbf{1.59  $\pm$ 0.30}  \\
\bottomrule
\end{tabular}
\caption{}
\label{tab:best_losses}
\end{table}

